Faster Approximation Algorithms for Parameterized Graph Clustering and Edge Labeling

Graph clustering is a fundamental task in network analysis where the goal is to detect sets of nodes that are well-connected to each other but sparsely connected to the rest of the graph. We present faster approximation algorithms for an NP-hard parameterized clustering framework called LambdaCC, which is governed by a tunable resolution parameter and generalizes many other clustering objectives such as modularity, sparsest cut, and cluster deletion. Previous LambdaCC algorithms are either heuristics with no approximation guarantees, or computationally expensive approximation algorithms. We provide fast new approximation algorithms that can be made purely combinatorial. These rely on a new parameterized edge labeling problem we introduce that generalizes previous edge labeling problems that are based on the principle of strong triadic closure and are of independent interest in social network analysis. Our methods are orders of magnitude more scalable than previous approximation algorithms and our lower bounds allow us to obtain a posteriori approximation guarantees for previous heuristics that have no approximation guarantees of their own.

==> arxiv/preamble.tex <==
% Packages and macros go here
\usepackage{amsfonts}
\usepackage{enumitem}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
\usepackage{mathtools}
% \usepackage{subfigure}
% \usepackage{graphicx}
% % \usepackage{subcaption}
% \usepackage{subfig}
% \usepackage{cite}
\usepackage{graphicx} % ,subcaption
% \usepackage{subfig}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}


\newcommand{\cut}{\textbf{cut}}
\newcommand{\dircut}{\textbf{dircut}}
\newcommand{\vol}{\textbf{vol}}
\newcommand{\gvol}{\textbf{gvol}}

\newcommand{\lamcc}{\textbf{CC}_{(\lambda)}}
\newcommand{\lamstc}{\textbf{STC}_{(\lambda)}}
\newcommand{\minstc}{\textsc{minSTC}}
\newcommand{\minstcp}{\textsc{minSTC+}}
\newcommand{\cheaper}{\emph{simplified}}

\providecommand{\mat}[1]{\boldsymbol{\mathrm{#1}}}%
\renewcommand{\vec}[1]{\boldsymbol{\mathrm{#1}}}



\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\minimum}{minimum}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\argmin}{argmin}
\providecommand{\subjectto}{\ensuremath{\text{subject to}}}

\providecommand{\eye}{\mat{I}}
\providecommand{\mA}{\ensuremath{\mat{A}}}
\providecommand{\mB}{\ensuremath{\mat{B}}}
\providecommand{\mC}{\ensuremath{\mat{C}}}
\providecommand{\mD}{\ensuremath{\mat{D}}}
\providecommand{\mE}{\ensuremath{\mat{E}}}
\providecommand{\mF}{\ensuremath{\mat{F}}}
\providecommand{\mG}{\ensuremath{\mat{G}}}
\providecommand{\mH}{\ensuremath{\mat{H}}}
\providecommand{\mI}{\ensuremath{\mat{I}}}
\providecommand{\mJ}{\ensuremath{\mat{J}}}
\providecommand{\mK}{\ensuremath{\mat{K}}}
\providecommand{\mL}{\ensuremath{\mat{L}}}
\providecommand{\mM}{\ensuremath{\mat{M}}}
\providecommand{\mN}{\ensuremath{\mat{N}}}
\providecommand{\mO}{\ensuremath{\mat{O}}}
\providecommand{\mP}{\ensuremath{\mat{P}}}
\providecommand{\mQ}{\ensuremath{\mat{Q}}}
\providecommand{\mR}{\ensuremath{\mat{R}}}
\providecommand{\mS}{\ensuremath{\mat{S}}}
\providecommand{\mT}{\ensuremath{\mat{T}}}
\providecommand{\mU}{\ensuremath{\mat{U}}}
\providecommand{\mV}{\ensuremath{\mat{V}}}
\providecommand{\mW}{\ensuremath{\mat{W}}}
\providecommand{\mX}{\ensuremath{\mat{X}}}
\providecommand{\mY}{\ensuremath{\mat{Y}}}
\providecommand{\mZ}{\ensuremath{\mat{Z}}}
\providecommand{\mLambda}{\ensuremath{\mat{\Lambda}}}
\providecommand{\mzero}{\ensuremath{\mat{0}}}

\providecommand{\ones}{\vec{e}}
\providecommand{\va}{\ensuremath{\vec{a}}}
\providecommand{\vb}{\ensuremath{\vec{b}}}
\providecommand{\vc}{\ensuremath{\vec{c}}}
\providecommand{\vd}{\ensuremath{\vec{d}}}
\providecommand{\ve}{\ensuremath{\vec{e}}}
\providecommand{\vf}{\ensuremath{\vec{f}}}
\providecommand{\vg}{\ensuremath{\vec{g}}}
\providecommand{\vh}{\ensuremath{\vec{h}}}
\providecommand{\vi}{\ensuremath{\vec{i}}}
\providecommand{\vj}{\ensuremath{\vec{j}}}
\providecommand{\vk}{\ensuremath{\vec{k}}}
\providecommand{\vl}{\ensuremath{\vec{l}}}
\providecommand{\vm}{\ensuremath{\vec{m}}}
\providecommand{\vn}{\ensuremath{\vec{n}}}
\providecommand{\vo}{\ensuremath{\vec{o}}}
\providecommand{\vp}{\ensuremath{\vec{p}}}
\providecommand{\vq}{\ensuremath{\vec{q}}}
\providecommand{\vr}{\ensuremath{\vec{r}}}
\providecommand{\vs}{\ensuremath{\vec{s}}}
\providecommand{\vt}{\ensuremath{\vec{t}}}
\providecommand{\vu}{\ensuremath{\vec{u}}}
\providecommand{\vv}{\ensuremath{\vec{v}}}
\providecommand{\vw}{\ensuremath{\vec{w}}}
\providecommand{\vx}{\ensuremath{\vec{x}}}
\providecommand{\vy}{\ensuremath{\vec{y}}}
\providecommand{\vz}{\ensuremath{\vec{z}}}

\newcommand{\hw}{\hat{w}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hm}{\hat{m}}
\newcommand{\hy}{\hat{y}}
\newcommand{\ha}{\hat{a}}
\newcommand{\hb}{\hat{b}}

\usepackage{amsthm}
\newtheorem{claim}{Claim}
\newtheorem{theorem}{Theorem}
\numberwithin{theorem}{section}
%\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{observation}{Observation}
\numberwithin{observation}{section}
\newtheorem{definition}{Definition}
\numberwithin{definition}{section}
\newtheorem{conjecture}{Conjecture}
\numberwithin{conjecture}{section}

==> arxiv/sections/introduction.tex <==

\section{Introduction}
% (Paragraph 1: graph clustering basics)
% *Graph clustering definition
% *Examples of applications
% *Typically cast as an optimization problem, often tied to statistical assumptions but not necessarily.
% *All strike a balance between two key goals, internal density and external sparsity.
% * Resolution parameter methods strike a balance between these two.

In network analysis, graph clustering is the task of partitioning a graph into well-connected sets of nodes (called communities, clusters, or modules), that are more densely connected to each other than they are to the rest of the graph~\cite{fortunato2016communitydetection}. 
%This task is also commonly known as \emph{community detection}, especially in social network analysis. 
This fundamental task has widespread applications across numerous domains, including detecting related genes in biological networks~\cite{shamir2004cluster,Ben-DorShamirYakhini1999}, finding communities in social networks~\cite{veldt2018correlation}, and image segmentation~\cite{wang2013scalable,ShiMalik2000}, to name only a few. A standard approach for finding clusters in a graph is to optimize some type of combinatorial objective function that encodes the quality of a clustering of nodes. Just as there are many different applications and reasons why one may with to partition the nodes of a graph into clusters, there are many different types of objective functions for graph clustering~\cite{newman2004modularity,ShiMalik2000,shamir2004cluster,bohlin2014community}, all of which strike a different balance between finding finding clusters with dense internal connections, and sparse connections between clusters. [add explanation about]


(Paragraph 2: the research gap, existing limitation)

Been studied for a long time, but there is still a large theory-practice gap.

The objectives are NP-hard, so while objectives are often easy to define, actually developing algorithms that are guaranteed to solve those objectives well or find something that is near optimal is very challenging.

Many algorithms are purely heuristics, and come with not approximation guarantees.

On the other hand in the theory literature, there are many approximation algorithms for graph clustering objectives, producing a solution that comes within a multiplicative factor of optimal. However, in most circumstances, these are impractical, as they often rely on solving expensive convex relaxations (e.g., linear programming or semi-definite programming relaxations of NP-hard objectives).


(Paragraph 3: our focus on LambdaCC)


In our work we focus on the LambdaCC framework. One benefit of this objective is that it generalizes many other objectives. At the same time, it is amenable to approximation algorithms. This is because it's a special case of correlation clustering, a framework for clustering that has been studied extensively from the perspective of approximation algorithms. For any value of $\lambda \in (0,1)$, it has an $O(\log n)$ approximation. For $\lambda \geq 1/2$, an improved 3-approximation is possible. However, this framework suffers from the same theory practice gap that other clustering frameworks do. The LP-based approximations are very expensive, and while 


(Paragraph 4: Our contributions)

\paragraph{The present work: combinatorial approximation algorithms for parameterized graph clustering.}

We develop faster approximation algorithms for the LambdaCC framework that apply for a range of resolution parameters. Mirroring previous results, we focus on the setting where lambda is from 1/2 to 1, as this is the regime where constant factor approximations are known to be possible. This is also the regime where LabmdaCC interpolates between two existing objectives for clustering know as cluster editing and clustering deletion.

We first of all design a fast combinatorial approximation algorithm that returns a 6-approximation for any value of $\lambda \geq 1/2$, that runs in only $O(\sum d_v^2)$  (which is at most $O(EV)$ and typically far less) time. While this approximation factor is a factor of 2 worse that the best case for this setting, it is orders of magnitude faster than the previous approach, which requires solving an LP relaxation with $O(n^3)$ variables. Our second algorithm is an improved $7-2/\lambda$ approximation (which ranges from 3 to 5 as lambda goes to 1), This LP relaxation first of all has far fewer constraints (in practice we confirm that on real-world graphs it typically scales as blah rather than $O(n^3)$), so even when solving it with black-box LP solver it is far more efficient. Even more significantly, it is a covering LP, which means that there exist combinatorial algorithms for solving it. Furthermore, in numerical experiments we nearly always find that solving this cheaper relaxation actually can be certified as the optimal solution to the canonical relaxation, in which case we can use previous rounding techniques to guarantee a . In the small lambda regime, we also show how similar techniques can produce a $1+ 1/\lambda$ approximation. Although this is far worse than a constant factor, that is not surprising, given that this is known to have an $O(\log n)$ integrality gap. This also come very close to the $1/\lambda$ approximation previously developed by Gleich et al. that relies on solving and rounding canonical LP.

All of our approximation algorithms rely on a new connection between LambdaCC and an edge labeling problem that is related to the principle of strong triadic closure, a principle in social network analysis that posits that if two people share strong links to a mutual friend, then the are likely to share at least a connection to each other. This principled has inspired a line of research on strong triadic closure labeling problems, which label edges in a graph as weak, strong (or in some cases ``missing") in order to satisfy strong triadic closure. Previous research has shown that certain unweighted variants of this labeling problem are related to clustering objective cluster deletion and cluster editing (which are equivalent to LambdaCC when $\lambda = 1/2$ and $\lambda \approx 1$ respectively). Recently it was shown that solving lower bounds for these unweighted STC problems can be a useful step in designing faster approximation algorithms for cluster editing and cluster deletion. We generalize this strategy by defining a new parameterized Edge-labeling problems we call LambdaSTC, which provides new types of lower bounds for LambdaCC. We also provide a 3-approximation algorithm that applies to every value of 3. While these results on edge labeling are interesting in their own right, our primary interest is rounding lower bounds for STC in order to develop better approximation algorithms for LambdaCC. Finally, we demonstrate in numerical experiments that our algorithms our very effective and fast.


To summarize, we have the following contributions:

\begin{itemize}
\item  6 approximation
\item  $7- 2/\lambda$ approximation
\item  We introduce a new edge labeling problem called LambdaSTC which generalizes previous edge labeling problems, along with a 3-approximation guarantee
\item  In numerical experiments, we show that these approaches are orders of magnitude faster than previous techniques and far exceed their theoretical guarantees.
\end{itemize}


==> arxiv/sections/prelims.tex <==
\section{Preliminaries}
% In this section, we present the key concepts and notation used throughout the paper, providing a foundation for understanding the subsequent discussions and results.
% We start by defining the basic formulation of LambdaCC(Lambda Correlation Clustering)~\cite{veldt2018correlation,veldt2017unifying} framework as a special variant of correlation clustering, which allows for more nuanced clustering decisions based on edge weights. We then present the notion of strong triadic closure labeling and highlight its importance associated with achieving efficient clustering solutions. By establishing a solid understanding of these preliminary concepts, we can delve into the main contributions of our work and provide a comprehensive analysis of approximation methods.

This section provides the foundational concepts and notation used in the paper. It introduces the LambdaCC framework as a variant of correlation clustering and emphasizes the significance of strong triadic closure labeling for effective clustering. Understanding these concepts sets the stage for the subsequent analysis of approximation methods in graph clustering.

Graph clustering problem involves partitioning the vertices of a graph into clusters based on their connectivity patterns. The objective is to identify groups of vertices that are densely connected within clusters and sparsely connected between clusters. Throughout the paper, we consider a given undirected and  graph $G = (V, E)$, where $V$ represents the set of vertices and $E$ represents the set of edges. The problem aims at finding a partitioning of $V$ into disjoint subsets (clusters) such that each vertex belongs to only one cluster and edges within clusters are maximized while those between clusters are minimized. 



\subsection{The LambdaCC Framework}
% Introduce the LambdaCC framework, giving a formal definition and mentioning all the other problems it generalizes.
The primary goal of any graph partitioning problem is to optimize a clustering criterion that quantifies the quality of the obtained partitions. The LambdaCC objective provides such criterion by incorporating a parameter called $\lambda$. \textbf{LambdaCC clustering problem} is defined as follows - Given an unweighted graph $G = (V, E)$ and clustering parameter $\lambda \in (0,1)$, find a partitioning of the vertices V into clusters $C_1, C_2, ...$ such that the clustering solution correlates well with the edge weights, for a specific fixed  parameter $\lambda$.
The LambdaCC problem can be defined as follows:

\vspace{-1em}
\[\begin{aligned}
		\min_{\delta} \quad & \sum_{(i,j)\in E}(1-\lambda)(1-\delta_{ij}) + \sum_{(i,j)\notin E}\lambda\delta_{ij}\\
            \text{s.t.} \quad & \delta_{ij}= \begin{cases} 1, & \text{if } C[i] = C[j]\\
            0, & \text{otherwise}
            \end{cases}
            % & \delta_{ij} \in \{0,1\}\\
            % & \delta_{ik} \leq \delta_{ij}+\delta_{jk} 
	\end{aligned}\]
\vspace{-1em}

where $C[i]$ denotes the cluster for $i$, and $\delta_{ij}$ is a binary indicator for every node-pair such that $\delta_{ij}=1$ if $i$ and $j$ are clustered together and $0$ when they are separate. The penalty of clustering dissimilar nodes together is $\lambda$ whereas that of separating similar nodes is $(1-\lambda)$.

LambdaCC framework is motivated by various applications, including community detection, network analysis, and data clustering, where the strength of the connections and the desired level of separation between clusters can be controlled by $\lambda$. By adjusting its value, different trade-offs can be achieved between cluster separations and cluster cohesiveness, allowing flexibility in the clustering results. It thus generalizes several clustering objectives like modularity~\cite{newman2004modularity,newman2006modularity}, sparsest cut~\cite{arora2009scut}, cluster editing~\cite{shamir2004cluster,dehne2006cluster,bocker2013ceditsurvery} ,cluster deletion~\cite{gramm2003graph,shamir2004cluster} and maximum likelihood stochastic block model~\cite{holland1983stochastic,karrer2011stochastic,NIPS2008_8613985e}

\subsection{Correlation Clustering}
% Background on correlation clustering (definition, ILP formulation, LP relaxation, van Zuylen and Williams)

% Then give specifics on how LambdaCC is a special case of this more general problem, and how this leads to a 3-approximation for $\lambda \geq 1/2$ and other results (cite them).


% This is how we get approximation algorithms, by thinking of graph clustering as correlation clustering.
% The fact that each of the positive mistakes share a common penalty while every one of the negative mistakes share another common cost value is what makes this objective more amenable to approximation than the general weighted version of correlation clustering. The asymmetry in the penalties associated with the \emph{disagreements} While at the same time, the ability to tune the nature of these penalties by changing the $\lambda$ parameter makes the framework more general and  robust than the unweighted clustering versions.

The CC in LambdaCC stands for correlation clustering~\cite{BansalBlumChawla2004}. In the most general setting, an instance of weighted correlation clustering is given by a set of vertices $V$, along with two non-negative weights $(w_{ij}^+,w_{ij}^-)$ for each pair of pair of vertices $(i,j) \in {V \choose 2}$. These weights indicate how similar or dissimilar nodes $i$ and $j$ are from each other. If nodes $(i,j)$ are placed in the same cluster, this incurs a penalty of their weight $w_{ij}^-$ whereas if they are separated, a penalty of $w_{ij}^+$ is imposed (the degree to which they are similar or dissimilar). The objective is to partition the vertices in a way that minimizes the number of disagreements between pairs of vertices with respect to their edge weights. Formally, it can be represented as an integer linear progrram as follows:
\begin{equation}
	\begin{aligned} \label{eq:cc_ilp}
		\text{ min}\quad &  \sum_{(i,j)\in E}w_{ij}^+x_{ij} + \sum_{(i,j)\notin E}w_{ij}^-(1-x_{ij})\\
		\text{s.t} \quad &  x_{ij}\leq x_{ik}+x_{jk} \text{ for all } i,j,k\\
		& x_{ij}\in \{0,1\} \text{ for all } i,j   
	\end{aligned}
\end{equation}
where $x_{ij}$ is the distance variable between nodes $i,j$ such that $x_{ij} = 0$ means nodes $i$ and $j$ are clustered together, and $x_{ij} = 1$ means they are separated. This is known as the min-disagree objective for correlation clustering; another objective is to instead maximize the weight of \emph{agreements}, which is similar at optimality but different in terms of approximation. We focus in our work on the min-disagree objective.

Correlation clustering is an NP-hard problem in correlation clustering, and addressing it optimally is computationally demanding. To overcome this challenge, several approximation algorithms~\cite{AilonCharikarNewman2008,CharikarGuruswamiWirth2003,CharikarGuruswamiWirth2005,ChawlaMakarychevSchrammEtAl2015} have been proposed that rely on solving an LP relaxation of \ref{eq:cc_ilp}. Ailon et al.~\cite{AilonCharikarNewman2008} introduced a randomized PIVOT algorithm for the unweighted graph that works iteratively by selecting a random pivot vertex and grouping together the neighboring vertices connected by edges. This process is repeated until all vertices are assigned to clusters. This combinatorial algorithm gives a clustering with an expected cost at most three times the cost of the optimal solution. However, running PIVOT on the general instances of weighted correlation clustering can yield poor results.

\textbf{Van Zuylen and Williamson} ~\cite{vanzuylen2009deterministic} devised a more general and deterministic strategy of using PIVOT for a certain more general weighted correlation clustering problem. Instead of directly choosing a random pivot from the weighted graph, this technique relies on deriving a new graph $\hat{G}$ such that running PIVOT on this new graph will produce a solution that bounds the clustering objective on the number of disagreements. This method involves choosing a set of 'budgets' for every pair of vertices such their total value lower bounds the optimal clustering solution. The following theorem frames the conditions for constructing the derived graph and bounding the clustering solution.
\begin{theorem}\label{thm_2.1}
Given an instance of weighted correlation clustering defined by an input set of vertices $V$, a set of edge-weights $(w^+,w^-)$ and a set of budgets $\{b_{ij}\}$ for every node-pair $(i,j)$ where $i\neq j$, and given a graph $\hat{G} (V,\hat{E})$ for some $\alpha>0$ that satisfies the following conditions:

\begin{enumerate} 
		\item $w_{ij}^- \leq \alpha b_{ij}$ for all edges $(i,j) \in \hat{E}$, and \\
            $w_{ij}^+ \leq \alpha b_{ij}$ for all edges $(i,j) \notin \hat{E}$
		\item $w_{ij}^+ + w_{jk}^+ + w_{ik}^- \leq \alpha (b_{ij}+b_{jk}+b_{ik})$ For every triplet $\{i,j,k\}$ in $\hat{G}$ where $\{i,j\}\in \hat{E}, \{j,k\}\in \hat{E}, \{i,k\}\notin \hat{E}$
	\end{enumerate}
Applying PIVOT on the derived graph $\hat{G}$ will then return a clustering solution with an expected objective cost that is bounded by $\alpha\sum_{i<j}b_{ij}$.
\end{theorem}
Using this strategy, we can prove approximation results of algorithms that use PIVOT for different variants of correlation clustering. LambdaCC can be considered as a special weighted variant of correlation clustering
where only one of $\{w_{ij}^+, w_{ij}^-\}$ is non-negative (to indicate that the two nodes are \emph{either} similar \emph{or} dissimilar). Given an input graph $G(V,E)$ and parameter $\lambda$, LambdaCC assigns a weight for each pair of nodes $(i,j) \text{ where } i \neq j$ . The associated weights for neighboring nodes are defined as $(w_{ij}^+,w_{ij}^-) = (1-\lambda,0)$ whereas those for non-neighboring nodes are $(w_{ij}^+,w_{ij}^-) = (0,\lambda)$. This specific case of the more general correlation clustering problem can be represented as the following integer linear program

\begin{equation}
	\begin{aligned} \label{eq:lamcc_ilp}
		\text{ min}\quad &  \sum_{(i,j)\in E}(1-\lambda)x_{ij} + \sum_{(i,j)\notin E}\lambda(1-x_{ij})\\
		\text{s.t} \quad &  x_{ij}\leq x_{ik}+x_{jk} \text{ for all } i,j,k\\
		& x_{ij}\in \{0,1\} \text{ for all } i,j   
	\end{aligned}
\end{equation}

Since the integer linear programming (ILP) formulation (\ref{eq:lamcc_ilp}) is NP-hard,  Veldt et al.~\cite{veldt2018correlation} presented a 3-approximation algorithm for values of $\lambda \geq 1/2$ by rounding the linear programming (LP) relaxation of (\ref{eq:lamcc_ilp}).

In this paper, our focus is on developing faster approximation algorithms for the LambdaCC problem, both with and without using LP relaxations, specifically targeting values of $\lambda \geq 1/2$. For values of $\lambda < 1/2$, another study by Veldt et al. ~\cite{Veldt2018ccgen} demonstrated an integrality gap of $O(\log n)$ for certain small values of $\lambda$. Their research also revealed that as $\lambda$ decreases, the performance of approximation algorithms worsens, as indicated by the deteriorating parameter-dependent approximation guarantees.
Therefore, our aim is to explore improved approximation algorithms for the LambdaCC problem across a range of $\lambda$ values, with a particular emphasis on achieving faster computation times while maintaining good approximation quality.


\subsection{Strong Triadic Closure and Edge Labeling}
% We should convey the message here that understanding strong triadic closure and solving edge labeling problems are of independent interest in social network analysis, and our paper includes contributions of independent interest on this. Our primary interest, however, is in using edge labeling problems as a step in broader clustering frameworks. This section should cite some of the previous work on how special cases of correlation clustering (cluster deletion and editing) are related to edge labeling problems.


% This section highlights the independent significance of understanding strong triadic closure(STC) and solving edge labeling problems in social network analysis. While these topics have been extensively studied in previous research, our paper focuses on utilizing edge labeling problems as a crucial step within broader clustering frameworks. We explore the connections between special cases of correlation clustering, such as cluster deletion and editing, and edge labeling problems. By building upon existing research, our contributions extend the understanding and application of edge labeling methods in correlation clustering, demonstrating their practical significance in social network clustering.

% Strong triadic closure~\cite{easley2010networks,granovetter1973strength} highlights the tendency of connected nodes to form triangles or triads. In other words, if two nodes in a network are strongly connected to a common neighbor, there is a higher likelihood that they will also be atleast weakly connected to each other. Edge labeling problems~\cite{sintos2014using,gruttemeier2020relation,konstantinidis2018strong} using this property offer a way to assign labels to edges based on their relationships, enabling the identification of meaningful patterns and structures within networks.Prior research, as evidenced by studies such as Gruttemeier et al. ~\cite{gruttemeier2020relation}, Konstantinidis et al. ~\cite{konstantinidis2018strong}, Gruttemeier ~\cite{gruttemeierstrong} , has established a strong connection between solving strong triadic closure labeling and addressing two specific clustering problems: cluster editing and cluster deletion. Veldt ~\cite{veldt2022stc} further proposed novel techniques to round the lower bounds for STC labeling problems, offering approximate clustering solutions for these two problems. 

% Veldt ~\cite{veldt2022stc}  introduced novel techniques to approximate clustering solutions for these problems by rounding lower bounds for STC labeling.

Strong triadic closure ~\cite{easley2010networks,granovetter1973strength} is a network phenomenon where connected nodes tend to form triangles. In other words, if two nodes in a network are strongly connected to a common neighbor, there is a higher likelihood that they will also be atleast weakly connected to each other. Edge labeling problems~\cite{sintos2014using,gruttemeier2020relation,konstantinidis2018strong} utilize this property to assign labels based on relationships, revealing meaningful patterns in networks. Previous research~\cite{gruttemeier2020relation,konstantinidis2018strong,gruttemeierstrong} has linked strong triadic closure(STC) labeling to cluster editing and cluster deletion problems.  A \emph{strong triadic closure labeling} seeks to label every edge as \emph{weak} or \emph{strong}, and every non-edge as \emph{missing} or not, such that STC property holds for every open triangle in $G$. In graph $G = (V, E)$, a triplet of vertices $(i,j,k)$ forms an \textbf{open triangle} centered at $j$ if the vertex pairs $(i,j)$ and $(i,k)$ are edges (i.e., in $E$) while $(i,k)$ is not. We use notations $\mathcal{T}$ to denote the set of all triplets that define an open triangle, and $\mathcal{T}_j$ to specifically refer to an open triangle centered at node $j$. 

\emph{Minimum weakness strong triadic closure with edge additions} (\textsc{minSTC+}) involves labeling existing edges as weak or strong, while allowing for the addition of weak edges between non-adjacent nodes in the graph. This can be interpreted as considering certain edges as "\emph{missing} connections" that were not initially observed. It satisfies the STC principle for an open triangle which posits that at least one of these connections is weak, or else $(i, k)$ would also be a \emph{missing} connection.The objective is to generate a labeling called STC+ labeling that minimizes the number of weak as well as missing edges while maintaining the STC property. Its integer formulation is 

\begin{equation}
	\label{minstc+}
	\begin{array}{lll}
		\min & \displaystyle{\sum_{(i,j) \in {V \choose 2}}} z_{ij} &\\
		\text{s.t. } & z_{ij} + z_{jk} + z_{ik} \geq 1 &\text{ if $(i,j,k) \in \mathcal{T}_j$}\\
		&  z_{ij} \in \{0,1\} &\text{ for $(i,j) \in {V \choose 2}$}.
	\end{array}		
\end{equation}
where labeling edges as weak ($(i,j)\in E$ and $z_{ij}=1$) and missing ($(i,j)\notin E$ and $z_{ij}=1$) yields a feasible STC+ labeling with a smallest number of added missing edges $E_{miss}$ and weak edges $E_{weak} \subseteq E$.

% \textbf{\textsc{minSTC} and cluster deletion}
\emph{ Minimum weakness strong triadic closure} (\textsc{minSTC}) involves assigning labels to existing edges in a network in a way that minimizes the number of weak edges while still satisfying the STC property.It can be cast as in integer program as follows:
\begin{equation}
	\label{minstc}
	\begin{array}{lll}
		\min & \sum_{(i,j) \in E} z_{ij} &\\
		\text{s.t. } & z_{ij} + z_{jk} \geq 1 &\text{ if $(i,j,k) \in \mathcal{T}_j$}\\
		&  z_{ij} \in \{0,1\} &\text{ for all $(i,j) \in E$}.
	\end{array}		
\end{equation}
where $z_{ij}$ is the indicator variable for labeling edges as weak($z_{ij}=1$) or not. 
\textsc{minSTC} can be considered as a cheaper form of relaxation for the \emph{cluster deletion} NP-hard problem. Cluster deletion(CD) aims to minimize the number of edge deletions in order to transform a graph into a collection of disjoint cliques. \textsc{minSTc} with an additional set of constraints $z_{ij}+z_{jk} \ge z_{ik}$ for every triplet of nodes ${i,j,k}$ forming a triangle in $G$, and a convenient change of variables leads to the cluster deletion(CD) integer problem. A feasible solution to CD thus corresponds to a feasible solution to \textsc{minSTC}, with the labeling that serves as a lower bound for the clustering objective. Rounding the lower bound labeling using \ref{thm_2.1} achieves a 2-approximate solution to the CD problem.




% \textbf{\textsc{minSTC+} and cluster editing}

 \textsc{minTSC+} presents a more cost-effective relaxation for the \emph{cluster editing}(CE) problem that aims to minimize the required edge additions or deletions to transform a graph $G$ into a collection of disjoint cliques. Similar to \textsc{minSTC}, an STC+ labeling lower bounds the CE problem an can be rounded to obtain a 3-approximation clustering solution.


 %  Clustering an open triangle in any manner will always incur a penalty by either grouping dissimilar nodes or separating similar nodes. Our work explores leveraging open triangle lower bounds to develop faster approximation algorithms for the more generalized LambdaCC objective.




